Ray-tracing for coordinate knowledge in the JWST Integrated Science Instrument Module

Optical alignment and testing of the Integrated Science Instrument Module of the James Webb Space Telescope is underway. We describe the Optical Telescope Element Simulator used to feed the science instruments with point images of precisely known location and chief ray pointing, at appropriate wavelengths and flux levels, in vacuum and at operating temperature. The simulator's capabilities include a number of devices for in situ monitoring of source flux, wavefront error, pupil illumination, image position and chief ray angle. Taken together, these functions become a fascinating example of how the first order properties and constructs of an optical design (coordinate systems, image surface and pupil location) acquire measurable meaning in a real system. We illustrate these functions with experimental data, and describe the ray tracing system used to provide both pointing control during operation and analysis support subsequently. Prescription management takes the form of optimization and fitting. Our core tools employ a matrix/vector ray tracing model which proves broadly useful in optical engineering problems. We spell out its mathematical basis, and illustrate its use in ray tracing plane mirror systems relevant to optical metrology such as a pentaprism and corner cube.

==> figures/preamble.bak.tex <==
%Inkscape TexText preamble
\usepackage{/media/DONGLE/data/Derek/Optics/papers/2014IODC_OSIM/manuscript/StyleGuide/osameet2}
\usepackage{ae}	%per OSA style guide, use ae to get computer modern fonts.  As of 2014/03/22, times fonts seem not to handle bold math notation.
\IfFileExists{mathpazo.sty}{\RequirePackage[osf,sc]{mathpazo}}{}
\usepackage{amsmath}                %AMS-LaTeX for advanced math typesetting features.  loaded by ua-thesis
\usepackage{amsfonts}   % for math typesetting commands like \mathbb
\usepackage{bm}	%enhanced bold math symbol support
\usepackage{bbm}	%enhanced blackboard bold (doublestruck) math symbol support
\newcommand{\acr}[1]{\textsc{\small{#1}}}    % typesetting for acronyms
\newcommand{\vctr}[1]{\ensuremath{\boldsymbol{#1}}}        %  notation for a vector


==> figures/preamble.tex <==
%Inkscape TexText preamble
%\usepackage{/media/DONGLE/data/Derek/Optics/papers/2014IODC_OSIM/manuscript/StyleGuide/osameet2}
%\usepackage{ae}	%per OSA style guide, use ae to get computer modern fonts.  As of 2014/03/22, times fonts seem not to handle bold math notation.
%\IfFileExists{mathpazo.sty}{\RequirePackage[osf,sc]{mathpazo}}{}
\usepackage{amsmath}                %AMS-LaTeX for advanced math typesetting features.  loaded by ua-thesis
\usepackage{amsfonts}   % for math typesetting commands like \mathbb
\usepackage{bm}	%enhanced bold math symbol support
\usepackage{bbm}	%enhanced blackboard bold (doublestruck) math symbol support
\newcommand{\acr}[1]{\textsc{\small{#1}}}    % typesetting for acronyms
\newcommand{\vctr}[1]{\ensuremath{\boldsymbol{#1}}}        %  notation for a vector

